Observation of $e^+e^-\to\eta\Upsilon(2S)$ and search for $e^+e^-\to\eta\Upsilon(1S),~\gamma X_b$ at $\sqrt{s}$ near 10.75 GeV

We present an analysis of the processes $e^{+}e^{-}\to\eta\Upsilon(1S)$, $\eta\Upsilon(2S)$, and $\gamma X_b$ with $X_b\to\pi^+\pi^-\chi_{bJ},~\chi_{bJ}\to\gamma\Upsilon(1S)$ $(J=1,~2)$ reconstructed from $\gamma\gamma\pi^+\pi^-\ell^+\ell^-~(\ell=e,~\mu)$ final states in $19.6\rm~\rm fb^{-1}$ of Belle II data collected at four energy points near the peak of the $\Upsilon(10753)$ resonance. Here, $X_b$ is a hypothetical bottomonium-sector partner of the $X(3872)$. In the process $e^{+}e^{-} \to \eta \Upsilon(2S)$, we observe a signal with a significance that exceeds $6.0\sigma$. Based on an analysis of the Born cross-section, the hypothesis that these events are associated solely with the production of the $\Upsilon(5S)$ or $\Upsilon(10753)$ resonances is rejected at the level of 3.6$\sigma$. This suggests that the observed events are more likely to arise from a new state near the $B^{*}\bar{B}^{*}$ threshold or from a substantial continuum production. No significant signal is observed for $e^{+}e^{-}\to\eta\Upsilon(1S)$ or $\gamma X_b$. Upper limits on the Born cross sections for the processes $e^{+}e^{-}\to\eta\Upsilon(1S)$ and $e^{+}e^{-}\to\gamma X_b$ with $X_b\to\pi^+\pi^-\chi_{bJ}$ are determined.

==> definitions.tex <==
% Packages
\usepackage{graphicx} % Include figure files
\usepackage{epstopdf} % Allow to include eps files
\usepackage{dcolumn} % Align table columns on decimal point
\usepackage{xcolor} % Color support
\usepackage{amssymb} % Extended symbol collection
\usepackage{hyperref} % Generate pdfs with hyperlinks
\usepackage[utf8]{inputenc} % Allow UTF8 characters
\usepackage[english]{babel} % All publications are in English
%\usepackage[displaymath, mathlines]{lineno} % Line numbers for drafts
\usepackage{blindtext} % For testing
\usepackage{bashful}
\usepackage{siunitx}
\usepackage[italic]{hepnames}
\usepackage{caption}
\usepackage{transparent}
\usepackage{helvet}
%\captionsetup{justification = raggedright, singlelinecheck = false}
\captionsetup{font=small, justification = raggedright, singlelinecheck = false}              
\usepackage{subcaption}
\usepackage{tikz}
\usepackage{tabularx}
\usepackage{amsmath}
\usepackage{orcidlink} % for ORCIDs in author list
\usepackage{lineno}
% Configuration


\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% THE NAME OF THE COLLABORATION %%%%
\def\belletwo {Belle~II }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace}
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}


\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\LL     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
%% \num conflicts with siunitx
% \def\num        {\ensuremath{\nu_\mu}\xspace}
% \def\numb       {\ensuremath{\nub_\mu}\xspace}
% \def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}
\def\pipipi{\ensuremath{\pi^+\pi^-\pi^0}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace}
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace}
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}
\def\Ddoublestar {\ensuremath{D^{**}}\xspace}
\def\Dzstar  {\ensuremath{D_{0}^{*}}\xspace}
\def\Done  {\ensuremath{D_{1}}\xspace}
\def\Doneprime  {\ensuremath{D'_{1}}\xspace}
\def\Dtwostar  {\ensuremath{D_{2}^{*}}\xspace}

\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace}
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\SixS  {\Y6S}

\def\chic#1{\ensuremath{\chi_{c#1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}

\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}


\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

%%%%%%%%%%%%%%%%
%% R(Xemu) analysis
%%%%%%%%%%%%%%%%

% define own units for siunitx
% barn was built-in but is deprecated in latest siunitx versions, so we have to define it ourselves
\DeclareSIUnit\clight{\text{\ensuremath{c}}}
\DeclareSIUnit\barn{b}
\DeclareSIUnit\b{\barn}
\DeclareSIUnit\fb{\femto\barn}
\DeclareSIUnit\invfb{\per\femto\barn}
\DeclareSIUnit\ab{\atto\barn}
\DeclareSIUnit\invab{\per\atto\barn}
\DeclareSIUnit\gev{\GeV}
\DeclareSIUnit\gevc{\GeV\per\clight}
\DeclareSIUnit\gevcc{\GeV\per\clight\squared}


% General stuff
\newcommand*{\btag}{\ensuremath{B_\text{tag}}\xspace}
\newcommand*{\bsig}{\ensuremath{B_\text{sig}}\xspace}
\newcommand{\pell}{\ensuremath{p_{\ell}^{B}}\xspace}
\newcommand*{\plab}{\ensuremath{p^{\mathrm{lab}}}\xspace}
\newcommand*{\thetalab}{\ensuremath{\theta^{\mathrm{lab}}}\xspace}
\newcommand{\sigprob}{\ensuremath{\mathcal{P}_\text{FEI}}\xspace}
\newcommand{\mbc}{\ensuremath{M_{\textrm{bc}}}\xspace}
\newcommand{\deltae}{\ensuremath{\Delta E}\xspace}
\newcommand{\lumion}{\ensuremath{\SI{189}{\per\femto\barn}}\xspace}
\newcommand{\lumioff}{\ensuremath{\SI{18}{\per\femto\barn}}\xspace}
\newcommand{\FEI}{\texttt{FEI}\xspace}
% R ratios and branching fractions.
\newcommand{\RXemu}{\ensuremath{R(X_{e/\mu})}\xspace}
\newcommand{\RXemufid}{\ensuremath{R(X_{e/\mu}\mid p_{\ell}^{B}>1.3\,\gevc)}\xspace}
\newcommand{\BtoXtaunu}{\ensuremath{B\to \, X \, \tau \, \nu}\xspace}
\newcommand{\BtoXellnu}{\ensuremath{B\to X \, \ell \, \nu}\xspace}
\newcommand{\BtoXenu}{\ensuremath{B\to X \, e \, \nu}\xspace}
\newcommand{\BFXenu}{\ensuremath{\mathcal{B}(\BtoXenu)}\xspace}
\newcommand{\BtoXmunu}{\ensuremath{B\to X \, \mu \, \nu}\xspace}
\newcommand{\BFXmunu}{\ensuremath{\mathcal{B}(\BtoXmunu)}\xspace}
\newcommand*{\xclnu}{\ensuremath{X_c \, \ell \, \nu}\xspace}
\newcommand{\btoclnu}{\ensuremath{b \to c \, \ell \, \nu}\xspace}
\newcommand{\btoulnu}{\ensuremath{b \to u \, \ell \, \nu}\xspace}
% D, D* modes
\newcommand{\bdlnu}{\ensuremath{B \to D \, \ell\,\nu}\xspace}
\newcommand{\bdslnu}{\ensuremath{B \to D^* \, \ell\,\nu}\xspace}
\newcommand{\bdanddslnu}{\ensuremath{B \to D^{(*)} \, \ell\,\nu}\xspace}
\newcommand{\bdenu}{\ensuremath{B \to D \, e\,\nu}\xspace}
\newcommand{\bdsenu}{\ensuremath{B \to D^* \, e\,\nu}\xspace}
\newcommand{\bdmunu}{\ensuremath{B \to D \, \mu\,\nu}\xspace}
\newcommand{\bdsmunu}{\ensuremath{B \to D^* \, \mu\,\nu}\xspace}
\newcommand{\bsdlnu}{\ensuremath{B_s \to D_s \, \ell\,\nu}\xspace}
\newcommand{\bsdslnu}{\ensuremath{B_s \to D^*_s \, \ell\,\nu}\xspace}
\newcommand{\bpDlnu}{\ensuremath{B^+ \to \overline D^0 \, \ell\,\nu}\xspace}
% D** modes
\newcommand{\bddslnu}{\ensuremath{B \to D^{**} \, \ell \,\nu}\xspace}
\newcommand{\bddsenu}{\ensuremath{B \to D^{**} \, e\,\nu}\xspace}
\newcommand{\bddsmunu}{\ensuremath{B \to D^{**} \, \mu\,\nu}\xspace}
\newcommand{\bdonelnu}{\ensuremath{B \to D_1 \, \ell\,\nu}\xspace}
\newcommand{\bdstwolnu}{\ensuremath{B \to D^*_2 \, \ell\,\nu}\xspace}
\newcommand{\bdszerolnu}{\ensuremath{B \to D^*_0 \, \ell\,\nu}\xspace}
\newcommand{\bdoneprimelnu}{\ensuremath{B \to D'_1 \, \ell\,\nu}\xspace}
\newcommand{\bdtwoSlnu}{\ensuremath{B \to D_{2S} \, \ell\,\nu}\xspace}
\newcommand{\bdstwoSlnu}{\ensuremath{B \to D^{*}_{2S} \, \ell\,\nu}\xspace}
% gap modes
\newcommand{\bdanddspipilnu}{\ensuremath{B \to D^{(*)}\,\pi\,\pi\,\ell\,\nu}\xspace}
\newcommand{\bdanddsetalnu}{\ensuremath{B \to D^{(*)}\,\eta\,\ell\,\nu}\xspace}
% LID calibration channels
\def\kspipi         {\ensuremath{K_{\rm S}^0\to\pi^+\pi^-}\xspace}
\def\jpsimumu       {\ensuremath{\jpsi \to \mup\mun}\xspace}
\def\jpsiee         {\ensuremath{\jpsi \to \ep\en}\xspace}
\def\jpsill         {\ensuremath{\jpsi \to \ell^+\ell^-}\xspace}
\def\LL             {\ensuremath{\ell^+\ell^-}\xspace}
\def\eegamma        {\ensuremath{\ep\en \to \ep\en (\gamma)}\xspace}
\def\mumugamma      {\ensuremath{\ep\en \to \mup\mun\gamma}\xspace}
\def\llgamma        {\ensuremath{\ep\en \to \ell^+\ell^-(\gamma)}\xspace}
\def\eeee           {\ensuremath{\ep\en \to (\ep\en)\ep\en}\xspace}
\def\eemumu         {\ensuremath{\ep\en \to (\ep\en)\mup\mun}\xspace}
\def\eell           {\ensuremath{\ep\en \to (\ep\en)\ell^+\ell^-}\xspace}
\def\eepipi         {\ensuremath{\ep\en \to (\ep\en)\pi^+\pi^-}\xspace}
\def\dstardkpipi    {\ensuremath{D^{*+}\to D^0(\to K^-\pi^+)\pi^+}\xspace}
\def\taupair        {\ensuremath{\ep\en\to \tau^{\pm}(\text{1-prong})\tau^{\mp}(\text{3-prong})}\xspace}
\def\ups        {\ensuremath{\Upsilon}\xspace}
% CS quantities
%\newcommand*{\scaleoffres}{\ensuremath{c_\textrm{off-res}}\xspace}
%\newcommand*{\ecmsoffres}{\ensuremath{\sqrt{s}_\textrm{off-res}}\xspace}
%\newcommand*{\ecmsonres}{\ensuremath{\sqrt{s}_{\FourS}}\xspace}


